TDEFSI: Theory Guided Deep Learning Based Epidemic Forecasting with Synthetic Information

Influenza-like illness (ILI) places a heavy social and economic burden on our society. Traditionally, ILI surveillance data is updated weekly and provided at a spatially coarse resolution. Producing timely and reliable high-resolution spatiotemporal forecasts for ILI is crucial for local preparedness and optimal interventions. We present TDEFSI (Theory Guided Deep Learning Based Epidemic Forecasting with Synthetic Information), an epidemic forecasting framework that integrates the strengths of deep neural networks and high-resolution simulations of epidemic processes over networks. TDEFSI yields accurate high-resolution spatiotemporal forecasts using low-resolution time series data. During the training phase, TDEFSI uses high-resolution simulations of epidemics that explicitly model spatial and social heterogeneity inherent in urban regions as one component of training data. We train a two-branch recurrent neural network model to take both within-season and between-season low-resolution observations as features, and output high-resolution detailed forecasts. The resulting forecasts are not just driven by observed data but also capture the intricate social, demographic and geographic attributes of specific urban regions and mathematical theories of disease propagation over networks. We focus on forecasting the incidence of ILI and evaluate TDEFSI's performance using synthetic and real-world testing datasets at the state and county levels in the USA. The results show that, at the state level, our method achieves comparable/better performance than several state-of-the-art methods. At the county level, TDEFSI outperforms the other methods. The proposed method can be applied to other infectious diseases as well.

==> sections/subsections/exp-performance-real.tex <==
\subsection{Performance on Real Seasonal ILI Testing Dataset}
\label{subsec:realtest}
\subsubsection{Performance of Flat-resolution Forecasting}
We forecast state level ILI incidence for VA, 2017-2018 and NJ, 2017-2018 using TDEFSI models and comparison methods. 
Figure~\ref{fig:state2017} shows the forecasting performance on RMSE, MAPE, PCORR for (a) VA and (b) NJ. 
($i$) \textit{Performance on RMSE (left column of Figure~\ref{fig:state2017})}:
In VA, TDEFSI, TDEFSI-L, TDEFSI-RDENSE, SARIMA, ARGO, and LSTM achieve similar performance that is better than EpiFast and AdapLSTM. 
%TDEFSI-L achieves the best performance followed by TDEFSI, SARIMA with the horizon less than 3, while TDEFSI, TDEFSI-RDENSE, and LSTM achieve better performance than others as the horizon increases.
In NJ, TDEFSI and its variants consistently outperform others across the horizon, with an
average of $15\%$-$64\%$ improvement in terms of RMSE.
($ii$) \textit{Performance on MAPE (middle column of Figure~\ref{fig:state2017})}:
In VA, ARGO performs the best overall among all methods except with horizon 1 where TDEFSI and its variants and SARIMA perform better than ARGO.
In NJ, TDEFSI achieves the best performance closely followed by TDEFSI-RDENSE. 
($iii$) \textit{Performance on PCORR (right column of Figure~\ref{fig:state2017})}:
In VA, overall, TDEFSI and its variants, ARGO, SARIMA, and LSTM have similar performance, while TDEFSI-L performs  slightly better than the others.
In NJ, TDEFSI outperforms others on Pearson correlation (i.e. around 0.96 with horizon 1)  which on average has $20\%$-$100\%$ improvement \comr{(computed as v = (A-B)/B, i.e. A has v improvement compared with B)} compared with others, followed by TDEFSI-L, TDEFSI-RDENSE, and ARGO.

Figure~\ref{fig:state2017week} shows the \emph{temporal} state level model performance measured using MAPE: 
%(a) Performance for VA, 2017-2018 and (b) Performance for NJ, 2017-2018. 
%We only show MAPE because RMSE is not compatible across temporal dimension and PCORR is not quite meaningful for only ten horizon data points. 
The x-axis denotes $ew$ number, the value is averaged on ten horizons. A log y-scale is used. The black vertical line marks the peak week of the season in the state. We observe that these models perform quite differently around the beginning and the end of a season, while they have similar performance in weeks near the peak. The performance of EpiFast and AdapLSTM is unstable through the season. In VA, ARGO performs very well at the start and end period of the season, while in NJ, TDEFSI performs fairly well across all weeks, which is consistent with the observations from 
Figure~\ref{fig:vastate2017} and ~\ref{fig:njstate2017}.

The above discussion can be summarized in three observations:  
\begin{itemize}
    \item 
Our TDEFSI and its variants achieve comparable/better performance than the other methods on the state level ILI forecasting. 
\item 
The methods of EpiFast and AdapLSTM do not perform well for both states in terms of either RMSE or MAPE in our experiments. 
\item
LSTM is not robust between different states on all three metrics;  see Section~\ref{subsec:discussion}
for additional explanation.
\end{itemize}


\begin{figure}[t]
\centering
\subfloat[VA, 2017-2018]{\label{fig:vastate2017}\includegraphics[width=5.3in]{figures/va-state-2017-2018-new.png}}
\hfil
\subfloat[NJ, 2017-2018]{\label{fig:njstate2017}\includegraphics[width=5.3in]{figures/nj-state-2017-2018-new.png}}
\hfil
\caption{State level forecasting performance on real ILI testing dataset using RMSE, MAPE, PCORR. (a) Performance for VA, 2017-2018; (b) Performance for NJ, 2017-2018. TDEFSI and its variants, and all comparison methods are evaluated and compared. The x-axis denotes horizon number, the value is averaged on all weeks of the season. A log y-scale is used in RMSE and MAPE. TDEFSI and its variants achieve comparable/better performance than the baselines. }
\label{fig:state2017}
\end{figure}

\begin{figure}[t]
\centering
\subfloat[VA, 2017-2018]{\label{fig:vastate2017week}\includegraphics[width=2.5in]{figures/va-state-2017-2018-weekly.png}}
\hfil
\subfloat[NJ, 2017-2018]{\label{fig:njstate2017week}\includegraphics[width=2.5in]{figures/nj-state-2017-2018-weekly.png}}
\hfil
\caption{State level weekly forecasting performance on real ILI testing dataset using MAPE. (a) Performance for VA, 2017-2018; (b) Performance for NJ, 2017-2018. TDEFSI and its variants, and all comparison methods are evaluated and compared. The x-axis denotes $ew$ number, the value is averaged on ten horizons. A log y-scale is used. The black vertical line marks the peak week of the season in the state. }
\label{fig:state2017week}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=5.3in]{figures/nj-county-2017-2018-new.png}
\caption{County level forecasting performance on real ILI testing dataset using RMSE, MAPE, PCORR for NJ, 2017-2018. TDEFSI and its variants, and EpiFast are evaluated and compared in the results. The x-axis denotes horizon number, the value is averaged on all weeks of the season and across 21 counties in NJ. A log y-scale is used in RMSE and MAPE. TDEFSI and its variants significantly outperform EpiFast in RMSE.}
\label{fig:county2017}
\end{figure}

\begin{figure}[t]
\centering
\subfloat[NJ counties, RMSE-ratio]{\label{fig:ratermse}\includegraphics[width=1.7in]{figures/map_rmse.png}}
\hfil
\subfloat[NJ counties, MAPE-ratio]{\label{fig:ratemape}\includegraphics[width=1.7in]{figures/map_mape.png}}
\hfil
\subfloat[NJ counties, PCORR-ratio]{\label{fig:ratepcorr}\includegraphics[width=1.7in]{figures/map_pcorr.png}}
\hfil
\caption{Comparison of the county level spatial forecasting performance between TDEFSI and EpiFast for NJ, season 2017-2018. (a) RMSE-ratio; (b) MAPE-ratio; (c) PCORR-ratio. For each county in NJ, the ratio value of the county is computed using equations~\ref{equ:njrate}, which is the average value across horizons. A value larger than 1 (red color) means TDEFSI outperforms EpiFast, a value equal to 1 (white color) means they both perform equally, and a value smaller than 1 (green color) means EpiFast performs better than TDEFSI. The absolute magnitude of the value denotes the significance of the difference of the two models' performance. The comparison results exhibit that TDEFSI performs better than EpiFast in the counties located in the western NJ.}
\label{fig:njrate}
\end{figure}

\subsubsection{Performance of High-resolution Forecasting}
The performance of county level forecasts is evaluated on NJ 2017-2018. Due to the limitation on model resolution, only TDEFSI models and EpiFast can make meaningful county level forecasting. Thus we compare the performance among TDEFSI, TDEFSI-L, TDEFSI-RDENSE, and EpiFast.
In Figure~\ref{fig:county2017}, we show county level ILI forecasting performance on three metrics.  
The metric value of each node in the figure is the average value across 21 counties in NJ for each horizon. 
Our method consistently outperforms the comparison method EpiFast on RMSE (about $53\%$ improvement) and PCORR (about $60\%$ improvement).
Among TDEFSI variants, TDEFSI and TDEFSI-RDENSE perform better than TDEFSI-L on RMSE and PCORR, which indicates that the between-season observations are helpful for improving forecasting accuracy. 

However, for MAPE, EpiFast performs better than our method with a horizon of less than 4, while the error increases dramatically as the horizon increases.
%This implies that EpiFast can make good predictions on short-term county level forecasting. 
Noting equation~\ref{equ:mape}, MAPE is biased by small data values. From the ground truth of NJ county level ILI incidence, we find that many counties have small infection numbers during the whole flu season (most down to zero cases). 
\comr{The results indicate that ... (Need some explanation here.)}
Overall, our method significantly outperforms the comparison method on the county level forecasting. 

To better understand the results from a spatial perspective, we compare results between TDEFSI and EpiFast in Figure~\ref{fig:njrate}. For each county in NJ, we compare TDEFSI and EpiFast using a ratio value for each of three metrics defined as:
\begin{equation}
\begin{aligned}
RMSE-ratio &= \frac{\frac{1}{m}\sum_{i=1}^{m}RMSE_i(EpiFast)}{\frac{1}{m}\sum_{i=1}^{m}{RMSE_i(TDEFSI)}}\\
MAPE-ratio &= \frac{\frac{1}{m}\sum_{i=1}^{m}MAPE_i(EpiFast)}{\frac{1}{m}\sum_{i=1}^{m}{MAPE_i(TDEFSI)}}\\
PCORR-ratio &= \frac{\frac{1}{m}\sum_{i=1}^{m}PCORR_i(EpiFast)}{\frac{1}{m}\sum_{i=1}^{m}{PCORR_i(TDEFSI)}}
\end{aligned}
\label{equ:njrate}
\end{equation}
where $m$ is the number of horizons. For PCORR-ratio, we avoid negative values by adding 1. The ratio value is the average ratio across all horizons. For three kinds of ratios, a value larger than 1 means TDEFSI outperforms EpiFast, a value equal to 1 means they both have similar performance, and a value smaller than 1 means EpiFast performs better than TDEFSI. The absolute magnitude of the value denotes the significance of the difference of the two models' performance.

From Figure~\ref{fig:njrate} (a) RMSE-ratio, we observe that TDEFSI significantly outperforms EpiFast in all counties (all counties show red colors) especially in western areas of NJ state. In (b) MAPE-ratio, TDEFSI performs better than EpiFast in eleven out of twenty one counties, most of which are located in the west boundary of NJ state.  And (c) PCORR-ratio shows that TDEFSI constantly outperforms EpiFast in all counties (all in red colors). 
The comparison results exhibit that TDEFSI performs better than EpiFast in the counties located in the western NJ. In the flu forecasting experiment, EpiFast tries to find a model that most represents the state level observations from a large amount of models. However, the fitted model is usually local optimal due to the limitation of the searching algorithm and the computational efficiency. The fitted model is quite sensitive to the model parameter setting such as the initial cases and the places they start and so on. Thus, each local optimal model is supposed to perform differently with the others in discovering and forecasting spatiotemporal epidemic details of a given state. In our experiments, we run the searching algorithm once and then find a local optimal model which performs fairly well in the eastern NJ counties but not in the western NJ counties. If we run the searching algorithm again, we will find another local optimal model which might perform well in the western NJ counties. In TDEFSI model, the deep neural network model allows TDEFSI to learn a general pattern from many models. The learned model is an ensemble model which is not sensitive to disease parameter settings. Thus, TDEFSI is more robust than EpiFast in different runs of the flu forecasting experiment. 

 
\begin{figure}[t]
  \includegraphics[width=0.6\textwidth]{figures/va_nj_history.png}
  \caption{CDC surveillance ILI incidence of VA (blue dash line) and NJ (red dot line). It is observable that, for testing season 2017-2018, a similar epi-curve (i.e. similar curve shape and the peak size) occurs at season 2014-2015 in VA, while no similar seasons could be found in NJ.}
  \label{fig:history}
\end{figure}

\subsubsection{Discussion} \label{subsec:discussion}
In general, AdapLSTM and EpiFast do not perform very well in our experiments compared with other methods.
For AdapLSTM, weather features are considered for post adjustment of LSTM outputs. 
As stated in~\cite{venna2019novel}, the weather factors are estimated using time delays computed by apriori associations and selected by the largest confidence.
However, in our experiment, they all show very low confidences (less than 0.3).
This may cause arbitrary adjustment for predictions and  consequently poor performance.
For EpiFast, one possible reason is that we did not find a good estimate of the underlying disease model for a specific region and season due to the noisy CDC observations.
%As discussed in Section~\ref{sec:introduction}, if the observed data is too noisy then the learned underlying model tends to make predictions with large errors. 

ARGO performs slightly better on VA than on NJ. The possible reason is that about $80\%$ of the top 100 Google correlated terms for NJ are irrelevant to flu and most of them have zero frequencies, while the top 100 correlated terms for VA are of good quality. This will give ARGO a better performance on VA than on NJ.

Similarly, LSTM performs relatively better on VA than on NJ. 
\comr{One possible reason is that LSTM does not seem likely to make predictions outside the observed historical range. The model performance is closely related to whether a similar epicurve occurred in previous seasons.}
%One possible reason is that the trained models are overfitted due to the small size of the training dataset from CDC surveillance. 
%This is especially true for LSTM which needs to learn a large number of parameters. 
%With overfitting, the model performance depends on whether a similar epicurve occurred in previous seasons.
As shown in Figure~\ref{fig:history}, the epicurve of VA 2017-2018 is similar to that of VA 2014-2015. However, the epicurve of NJ 2017-2018 seems to be much higher than all previous ones.
On the contrary, TDEFSI models have stable performance on both VA and NJ. They manage to avoid overfitting through training on a large volume of synthetic training data. In addition, the simulated training dataset includes many realistic simulated patterns that are unseen in the real world, thus provides a better generalizability to our models.

As seen through the results, TDEFSI enables high-resolution forecasting that outperforms EpiFast. Meanwhile, it achieves comparable/better performance than the comparison methods at state level forecasting. And in our framework, the large volume of realistic simulated data allows us to train a more complex DNN model and reduces the risk of overfitting. Our experiments demonstrate that TDEFSI integrates the strengths of ANN methods and causal methods to improve epidemic forecasting.

==> sections/subsections/exp-what-if.tex <==
\subsection{What-if forecasting}
\label{subsec:what-if}
In this section, we are going to discuss a potential ability of TDEFSI framework -- \textit{what-if forecasting}. What-if forecasting means forecasts that can capture various what-if scenarios as epidemic is evolving. It is crucial when an unprecedented epidemic happens and consequently some public health interventions get involved during a flu season. The existing data-driven methods are hard to capture such patterns since they can only see historical observations. 
In our framework, high computing simulations of epidemic process allow us to incorporate multiple scenarios that are not really happening in current time but are of high possibility to happen in the future into the deep neural network model training. 
What-if scenarios can be any assumptions, such as emerging of the second virus strain during the season, temporary interventions like school closure or multiple vaccine schedules due to an intensive flu outbreak, etc. These scenarios can be involved in the epidemic simulations which will then generate new training data. The models trained on this data are able to capture the what-if scenarios leading to what-if forecasts, so helping the public health decision making and planning. 
What-if forecasting works as following using our framework:
\begin{itemize}
    \item Make an assumption $\zeta$
    \item Parameterize $\zeta$, $\Theta(\zeta)$, so that it can be applied to the epidemic simulation using casual models;
    \item Generate synthetic epi-curves using the simulations with $\Theta(\zeta)$;
    \item Expand training data with new generated curves;
    \item Train TDEFSI model on new training data;
    \item Make forecasting.
\end{itemize}
Note that multiple assumptions can stack in one simulation. We do not conduct experiments on what-if forecasting in this work, but the proposed framework shows promising future on this direction. 


==> tables/apdx-sim-cfg.tex <==
\begin{table*}[!t]
\centering
\caption{Simulation configuration. }
  \label{tab:sim_cfg}
  \begin{tabularx}{\linewidth}{lXX}
    \toprule
    Parameters & Description & Values\\
    \midrule
    ContactGraph & synthetic social contact network & state level contact social network \\
    ($P_E, p_I, \tau, N_I, I_V$) & user specified parameter space & sample from $\mathcal{P}$ \\
    AsymptomaticProbability & the probability of an infectious person without symptoms & 0.333 \\
    AsymptomaticFactor & scaling factor of infectivity of an asymptomatic case comparing with a symptomatic case & 0.53 \\
    SimulationDuration & simulation duration by days & 365 \\
    %ProbSymptomaticToHospital & the probability of a symptomatic person goes to hospital & 1 \\
    ProbDiagnoseSymptomatic & the probability of an infectious person is diagnosed as ILI & 0.6 \\
    %DiagnosedDuration & diagnose duration by days & 1 \\
    \bottomrule
\end{tabularx}
\begin{tablenotes}
  \small
  \item 
\end{tablenotes}
\end{table*}
